From Unstructured Data to In-Context Learning: Exploring What Tasks Can Be Learned and When

Large language models (LLMs) like transformers demonstrate impressive in-context learning (ICL) capabilities, allowing them to make predictions for new tasks based on prompt exemplars without parameter updates. While existing ICL theories often assume structured training data resembling ICL tasks (e.g., x-y pairs for linear regression), LLMs are typically trained unsupervised on unstructured text, such as web content, which lacks clear parallels to tasks like word analogy. To address this gap, we examine what enables ICL in models trained on unstructured data, focusing on critical sequence model requirements and training data structure. We find that many ICL capabilities can emerge simply from co-occurrence of semantically related word pairs in unstructured data; word analogy completion, for example, can provably arise purely through co-occurrence modeling, using classical language models like continuous bag of words (CBOW), without needing positional information or attention mechanisms. However, positional information becomes crucial for logic reasoning tasks requiring generalization to unseen tokens. Finally, we identify two cases where ICL fails: one in logic reasoning tasks that require generalizing to new, unseen patterns, and another in analogy completion where relevant word pairs appear only in fixed training positions. These findings suggest that LLMs' ICL abilities depend heavily on the structural elements within their training data.

==> attention-autompg.tex <==
% !TEX root = attention.tex

\begin{table}[ht]
\centering
\label{fig:auto-mpg-res}
\begin{tabular}{ccccccccccc}
\hline
 & LR & RF & GB & MLP  & CE & FT & TT & AI & TN & ATN (ours)\\ \hline
Accuracy & 0.657 & 0.721 & 0.657 & 0.700  & 0.764 & 0.707 & 0.707 & 0.364 & 0.600 & \textbf{0.793}\\ \hline
MSE & 0.343 & 0.279 & 0.343 & 0.300  & 0.236 & 0.293 & 0.293 & 0.636 & 0.486 & \textbf{0.207}\\ \hline
\end{tabular}
\caption{The proposed tabular extension of attention (ATN) achieves
superior performance as compared to all baselines. (Lower MSE and
higher accuracy is better.)}
\end{table}

==> attention-linear.tex <==
% !TEX root = attention.tex

\begin{table*}[t]
\centering

\label{table:acc}
\begin{tabular}{lllll}
\hline
\textbf{Accuracy}  & BERT  & GloVe & CBOW \\ \hline
Semantic  & 0.641 & 0.759 & 0.234 \\ \hline
Syntactic & 0.754 & 0.692 & 0.667 \\ \hline
Overall   & 0.727 & 0.708 & 0.563 \\ \hline
\end{tabular}
\qquad
% \label{table:cos}
\begin{tabular}{lllll}
\hline
\textbf{Cosine similarity}  & BERT  & GloVe  & CBOW \\ \hline
Semantic  & 0.500 & 0.600 & 0.504    \\ \hline
Syntactic & 0.610 & 0.610 & 0.582     \\ \hline
Overall   & 0.584 & 0.607 & 0.564     \\ \hline
\end{tabular}
\caption{Classical word embedding methods can achieve similar or
higher performance than attention-based model in word analogy tasks:
GloVe achieve higher or the same average cosine similarity than BERT
on both syntactic and semantic analogies; GloVe also outperforms BERT
in accuracy for semantic analogies. (Higher is better.)}
\end{table*}

==> attention-ood.tex <==
% !TEX root = attention.tex

\begin{table}[h!]
\centering
\label{fig:sim-res-acc}
% {\scriptsize
\begin{subtable}[t]{\linewidth}
\centering
\begin{tabular}{cccccc}
\hline
Param. $\backslash$ \textbf{Acc.} & LR & RF & GB & MLP & ATN \\ \hline
$(1, 0, 0.1)$ & 0.388 & 0.409 & \textbf{0.413} & 0.323 & 0.404 \\ 
$(1, 0, 0.9)$ & 0.313 & 0.298 & 0.350 & 0.237 & \textbf{0.389} \\ \hline
$(1, 0.5, 0.1)$ & 0.345 & 0.361 & \textbf{0.366} & 0.292 & 0.359 \\ 
$(1, 0.5, 0.9)$ & 0.270 & 0.253 & 0.299  & 0.202 & \textbf{0.306} \\ \hline
$(1, 1.5, 0.1)$ & 0.250 & 0.243 & \textbf{0.253} & 0.204 & 0.252 \\ 
$(1, 1.5, 0.9)$ & 0.169 & 0.158 & \textbf{0.172} & 0.142 & 0.170 \\ \hline
$(5, 0, 0.1)$ & 0.250 & 0.207 & 0.244 & 0.306 & \textbf{0.419} \\ 
$(5, 0, 0.9)$ & 0.162 & 0.150 & 0.156 & 0.169 & \textbf{0.392} \\ \hline
$(5, 0.5, 0.1)$ & 0.227 & 0.173 & 0.214 & 0.252 & \textbf{0.318} \\ 
$(5, 0.5, 0.9)$ & 0.154 & 0.133 & 0.153 & 0.151 & \textbf{0.269} \\ \hline
$(5, 1.5, 0.1)$ & 0.167 & 0.099 & 0.157 & 0.165 & \textbf{0.171} \\ 
$(5, 1.5, 0.9)$ & 0.125 & 0.108 & 0.114 & 0.118 & \textbf{0.133} \\ \hline
\end{tabular}
\caption{Accuracy}
\end{subtable}
\vspace{15pt}
\begin{subtable}[t]{\linewidth}
\centering
\begin{tabular}{cccccc}
\hline
Param. $\backslash$ \textbf{MSE} & LR & RF & GB & MLP & ATN \\ \hline
$(1, 0, 0.1)$ & 3.015 & \textbf{2.694} & 2.730 & 4.059 & 2.941 \\ 
$(1, 0, 0.9)$ & 5.163 & 9.331 & 4.855 & 7.911 & \textbf{3.078} \\ \hline
$(1, 0.5, 0.1)$ & 3.416 & 3.201 & \textbf{3.123} & 4.704 & 3.281 \\ 
$(1, 0.5, 0.9)$ & 5.955 & 10.106 & 6.070 & 8.123 & \textbf{4.465} \\ \hline
$(1, 1.5, 0.1)$ & 5.725 & 5.685 & \textbf{5.415} & 7.199 & 5.594 \\ 
$(1, 1.5, 0.9)$ & 8.942 & 12.340 & 9.837 & 9.874 & \textbf{7.339} \\ \hline
$(5, 0, 0.1)$ & 5.333 & 8.498 & 5.967 & 2.814 & \textbf{1.521} \\ 
$(5, 0, 0.9)$ & 5.674 & 10.101 & 8.858 & 7.842 & \textbf{1.633} \\ \hline
$(5, 0.5, 0.1)$ & 6.021 & 10.236 & 6.844 & 4.056 & \textbf{2.605} \\ 
$(5, 0.5, 0.9)$ & 6.118 & 10.427 & 8.283 & 7.884 & \textbf{2.355} \\ \hline
$(5, 1.5, 0.1)$ & 9.159 & 16.154 & 9.538 & \textbf{8.313} & 8.316 \\ 
$(5, 1.5, 0.9)$ & 8.410 & 10.409 & 10.110 & 9.966 & \textbf{6.501} \\ \hline
\end{tabular}
\caption{MSE}
\end{subtable}
% }
\caption{The proposed tabular extension of bidirectional attention
(ATN) achieves better or competitive accuracy and MSE than competing
methods, across all parameter settings. The parameter tuples indicate
different choices of $(n_c, \textrm{noise}, \textrm{corr})$.}
\end{table}

==> sec_related.tex <==
\section{Related work}
\label{app:rel-work}

Large language models (LLMs), such as transformers, are widely recognized for their outstanding performance in in-context learning (ICL) \citep{brown2020language}. ICL refers to the capability of LLMs to discern specific tasks and generate predictions based on input-output pairs (known as prompts) without needing any parameter updates. A multitude of studies have been dedicated to exploring this intriguing phenomenon from various theoretical and empirical perspectives. In this section, we provide a brief summary of some of these studies.

Some studies adopted a Bayesian approach to studying ICL. \citet{xie2021an} posited that ICL can be viewed as implicit Bayesian inference. They demonstrated that LLMs can infer a latent document-level concept for next-token prediction during pretraining and a shared latent concept across input-output pairs in an ICL prompt, under the assumption that documents are generated from hidden Markov models (HMMs). \citet{wang2023large} and \citet{zhang2023what} expanded on this idea by exploring more realistic latent variable models beyond HMMs. \citet{wang2023large} argued that large language models function as latent variable models, with latent variables containing task-related information being implicitly inferred. \citet{zhang2023what} showed that without updating the neural network parameters, ICL can be interpreted as Bayesian model averaging parameterized by the attention mechanism. \citet{ahuja2023in} provided empirical evidence that transformers behave like Bayesian predictors when performing ICL with linear and non-linear function classes. \citet{dalal2024the} proposed a Bayesian learning framework to understand ICL through the lens of text generation models represented by multinomial transition probability matrices. \citet{chiang2024understanding} proposed the pelican soup framework to explain ICL without relying on latent variable models. This framework incorporates concepts such as a common sense knowledge base, natural language classification, and meaning association, enabling the establishment of a loss bound for ICL that depends on the number of in-context examples.

\citet{garg2022what} formulated ICL as learning a specific function class $\mathcal{F}$ from prompts of the form $\left(x_1, f(x_1), \ldots, x_n, f(x_n), x_{n+1}\right)$ and their corresponding responses $f(x_{n+1})$. Here, $f \in \mathcal{F}$, where $\mathcal{F}$ is a function class. In this context, ICL refers to the capability of a transformer to output a number close to $g(y_{n+1})$ given a prompt of the form $\left(y_1, g(y_1), \ldots, y_n, g(x_n), y_{n+1}\right)$, where $g \in \mathcal{F}$. Many studies adopted this regression formulation of ICL, with some linking ICL to gradient descent. \citet{akyurek2022learning, oswald2023transformers}, and \citet{dai2023why} proved that transformers are capable of implementing gradient descent, which results in their ICL ability. \citet{bai2023transformers} established generalization bounds for ICL and proved that transformers can perform algorithm selection like statisticians. \citet{zhang2024trained} showed that the gradient flow dynamics of transformers converge to a global minimum that enables ICL. \citet{huang2023in} investigated the learning dynamics of single-layer softmax transformers trained via gradient descent to perform ICL on linear functions. \citet{ahn2024transformers} explored the optimization landscape of transformers and proved that the optimal parameters coincide with an iteration of preconditioned~gradient~descent. 

In a related exploration, \citet{li2023the} showed that softmax regression models learned through gradient descent are similar to transformers. \citet{ren2023in} related ICL with softmax transformers to contrastive learning, where the inference process of ICL can be viewed as a form of gradient descent. \citet{mahankali2023one} proved that minimizing the pretraining loss is equivalent to a step of gradient descent in single-layer linear transformers. \citet{vladymyrov2024linear} established that linear transformers execute a variant of preconditioned gradient descent by maintaining implicit linear models. On the other hand, some studies argued that the ICL ability of transformers cannot be attributed to gradient descent. \citet{fu2023transformers} showed that ICL for linear regression tasks arises from higher-order optimization techniques like iterative Newton's method rather than gradient descent. \citet{wibisono2023on} demonstrated that transformers can perform ICL on unstructured data that lack explicit input-output pairings, with softmax attention playing an important role especially when using a single attention layer. \citet{shen2023do} provided empirical evidence that the equivalence between gradient descent and ICL might not be applicable in real-world scenarios. \textcolor{red}{In contrast to these studies, our work provides a connection between ICL and classical language models like continuous bag of words (CBOW). Specifically, we show that ICL involving known input-output pairings can arise by modeling co-occurrence patterns via CBOW.}

Numerous studies focused on the pretraining aspects (e.g., data distribution and task diversity) of ICL. \citet{min2022rethinking} showed that the input-label mapping in the in-context examples does not significantly affect ICL performance. \citet{chan2022data} demonstrated that the ICL capabilities of transformers depend on the training data distributions and model features. \citet{kossen2023in} established that ICL considers in-context label information and is capable of learning entirely new tasks in-context. \citet{li2023finding} introduced an iterative algorithm designed to enhance ICL performance by selecting a small set of informative examples that effectively characterize the ICL task. \citet{qin2023in} proposed a method based on zero-shot chain-of-thought reasoning for selecting ICL examples, emphasizing the importance of choosing diverse examples that are strongly correlated with the test sample. \citet{han2023understanding} studied ICL by identifying a small subset of the pretraining data that support ICL via gradient-based methods. They discovered that this supportive pretraining data typically consist of more uncommon tokens and challenging examples, characterized by a small information gain from long-range context. \citet{peng2024revisiting} proposed a selection method for ICL demonstrations that are both data-dependent and model-dependent. \citet{van2024in} introduced a demonstration selection method that enhances ICL performance by analyzing the influences of training samples using influence functions.

In a similar vein, \citet{wu2023how} demonstrated that pretraining single-layer linear attention models for ICL on linear regression with a Gaussian prior can be effectively accomplished with a minimal number of independent tasks, regardless of task dimension. \citet{raventos2023pretraining} emphasized a task diversity threshold that differentiates the conditions under which transformers can successfully address unseen tasks. \citet{yadlowsky2023pretraining} attributed the impressive ICL capabilities of transformers to the diversity and range of data mixtures in their pretraining, rather than their inductive biases for generalizing to new tasks. \citet{ding2023causallm} compared the ICL performance of transformers trained with prefixLM (where in-context samples can attend to all tokens) versus causalLM (where in-context samples cannot attend to subsequent tokens), finding that the latter resulted in poorer ICL performance. \citet{chen2024parallel} discovered that the ICL capabilities of language models rely on the presence of pairs of phrases with similar structures within the same sentence. \citet{zhao2024noisyicl} proposed a calibration scheme that modifies model parameters by adding random noises, resulting in fairer and more confident predictions. \citet{abbas2024enhancing} demonstrated that the ICL predictions from transformer-based models often exhibit low confidence, as indicated by high Shannon entropy. To address this issue, they introduced a straightforward method that linearly calibrates output probabilities, independent of the model's weights or architecture. \textcolor{red}{Similar to these works, our work highlights  the importance of co-occurrence, positional information, and training data structure for ICL to arise.}


Other studies analyzed ICL from a learning theory perspective. \citet{hahn202a} proposed an information-theoretic bound that explains how ICL emerges from next-token prediction. \citet{wies2023the} derived a PAC-type framework for ICL and finite-sample complexity results. \citet{jeon2024an} introduced a novel information-theoretic view of meta-learning (including ICL), allowing for the decomposition of errors into three components. They proved that in ICL, the errors decrease as the number of examples or sequence length increase. Other studies focus on the mechanistic interpretability component of ICL. \citet{olsson2022in} argued that transformers can develop induction heads that are able to complete token sequences such as [A][B] $\cdots$ [A] $\rightarrow$ [B], leading to impressive ICL performance. \citet{bietti2023birth} examined a setup where tokens are generated from either global or context-specific bigram distributions to distinguish between global and in-context learning. They found that global learning occurs rapidly, while in-context learning is achieved gradually through the development of an induction head. \citet{ren2024identifying} identified semantic induction heads that increase the output logits of tail tokens when attending to head tokens, providing evidence that these heads could play a vital role in the emergence of ICL. \citet{yu2024how} showed that the ICL ability of transformers arises from the utilization of in-context heads, where each query and key matrix collaborate to learn the similarity between the input text and each demonstration example.

A number of works delved into specific data generating processes to provide insight into the emergence of ICL. \citet{bhattamishra2023understanding} examined the ICL ability of transformers by focusing on discrete functions. Specifically, they showed that transformers perform well on simpler tasks, struggle with more complex tasks, and can learn more efficiently when provided with examples that uniquely identify a task. \citet{guo2023how} investigated ICL in scenarios where each label is influenced by the input through a potentially complex yet constant representation function, coupled with a unique linear function for each instance. \citet{akyurek2024in} studied ICL of regular languages produced by random finite automata. They compared numerous neural sequence models and demonstrated that transformers significantly outperform RNN-based models because of their ability to develop \textit{n-gram heads}, which are a generalization of \textit{induction heads}. \citet{sander2024how} analyzed simple first-order autoregressive processes to gain insight into how transformers perform ICL to predict the next tokens. \textcolor{red}{On the other hand, our work focuses on data generating processes containing input-output relationship pairs or repeating token patterns to better understand several components that are crucial for ICL to occur from training on unstructured data.}


Some studies explored how different components of transformers affect their ICL abilities. \citet{ahuja2023a} compared the ICL performance of transformers and MLP-based architectures under distribution shifts. Their findings demonstrate that while both methods perform well in in-distribution ICL, transformers exhibit superior ICL performance when faced with mild distribution shifts. \citet{collins2024in} showed that softmax attention outperforms linear attention in ICL due to its ability to calibrate its attention window to the Lipschitzness of the pretraining tasks. \citet{xing2024benefits} focused on linear regression tasks to identify transformer components that enable ICL. They found that positional encoding is crucial, along with the use of multiple heads, multiple layers, and larger input dimensions. \citet{cui2024superiority} proved that multi-head attention outperforms single-head attention in various practical scenarios, including those with noisy labels and correlated features. \citet{chen2024training} investigated the ICL dynamics of a multi-head softmax attention model applied to multi-task linear regression. They proved the convergence of the gradient flow and observed the emergence of a \textit{task allocation} phenomenon, where each attention head specializes in a specific task.

Finally, several studies proposed various hypotheses on the emergence of ICL and provided theoretical justifications. \textcolor{red}{\citet{swaminathan2023schema} introduced clone-structured causal graphs (CSCGs) to explain how ICL can generalize to unseen sentences via a mechanism called rebinding.} \citet{li2023transformers} viewed ICL as an algorithm learning problem where a transformer implicitly constructs a hypothesis function at inference time. \citet{han2023explaining} argued that the ability of transformers  to execute ICL is attributable to their capacity to simulate kernel regression. \citet{singh2023the} explored the interaction between ICL and in-weights learning (IWL) using synthetic data designed to support both processes. They observed that ICL initially emerges, followed by a transient phase where it disappears and gives rise to IWL. \citet{yan2023understanding} studied ICL from the perspective that token co-occurrences play a crucial role in guiding the learning of surface patterns that facilitates ICL. \citet{abernethy2024a} showed that transformers can execute ICL by dividing a prompt into examples and labels, then employing sparse linear regression to deduce input-output relationships and generate predictions. \citet{lin2024dual} developed a probabilistic model that can simultaneously explain both task learning and task retrieval aspects of ICL. Here, task learning refers to the ability of language models to identify a task from in-context examples, while task retrieval pertains to their ability to locate the relevant task within the pretraining data.

